Small Language Models are Good Too: An Empirical Study of Zero-Shot Classification

This study is part of the debate on the efficiency of large versus small language models for text classification by prompting.We assess the performance of small language models in zero-shot text classification, challenging the prevailing dominance of large models.Across 15 datasets, our investigation benchmarks language models from 77M to 40B parameters using different architectures and scoring functions. Our findings reveal that small models can effectively classify texts, getting on par with or surpassing their larger counterparts.We developed and shared a comprehensive open-source repository that encapsulates our methodologies. This research underscores the notion that bigger isn't always better, suggesting that resource-efficient small models may offer viable solutions for specific data classification challenges.

==> assets/mean_per_scoring.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lr}
    \toprule
    strategy & Mean of Accuracy/F1 \\
    \midrule
    dcpmi & 0.387 \\
    pmi & 0.378 \\
    lm & 0.374 \\
    similarity & 0.298 \\
    \bottomrule
    \end{tabular}
    \caption{Mean of Accuracy \& F1 Scores by Scoring Functions}
\end{table}


==> results/per_architecture/tables/old/correlation_instruction_ft_metric_per_architecture.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lrl}
    \toprule
    dataset & statistic & pvalue \\
    \midrule
    seq2seq & 10.7985 & \textred{0.0010} \\
    causal & 0.2123 & 0.6450 \\
    \bottomrule
    \end{tabular}
    \caption{Kruskal-Wallis Statistics and P-values Indicating the Relationship Between Acc/F1 and instruction\_ft variable Across Architectures}
\end{table}


==> results/per_architecture/tables/old/correlation_strategy_metric_per_architecture.tex <==
\begin{table}[h]
    \centering
    \caption{Kruskal-Wallis Statistics and P-values Indicating the Relationship Between Acc/F1 and strategy Across architectures}
    \begin{tabular}{lrl}
    \toprule
    dataset & statistic & pvalue \\
    \midrule
    seq2seq & 2.1983 & 0.3332 \\
    causal & 2.1602 & 0.3396 \\
    \bottomrule
    \end{tabular}
\end{table}


==> results/per_datasets/tables/old/correlation_architecture_metric.tex <==
\begin{table}[h]
\caption{Kruskal-Wallis Statistics and P-values Indicating the Relationship Between Acc/F1 and architecture Across Datasets}
\begin{tabular}{lrl}
\toprule
dataset & statistic & pvalue \\
\midrule
agnews & 0.0059 & 0.9390 \\
bbcnews & 1.0328 & 0.3095 \\
cdr & 1.6638 & 0.1971 \\
chemprot & 1.4385 & 0.2304 \\
ethos & 0.0212 & 0.8842 \\
financial\_phrasebank & 0.7038 & 0.4015 \\
imdb & 0.0298 & 0.8630 \\
semeval & 2.6098 & 0.1062 \\
sms & 6.4746 & \textred{0.0109} \\
spouse & 3.0273 & \textred{0.0819} \\
sst-2 & 0.0462 & 0.8298 \\
sst-5 & 0.3807 & 0.5372 \\
trec & 1.1907 & 0.2752 \\
yelp & 0.1059 & 0.7449 \\
youtube & 9.3581 & \textred{0.0022} \\
\end{tabular}
\end{table}


==> results/per_datasets/tables/old/correlation_instruction_ft_metric.tex <==
\begin{table}[h]
\caption{Kruskal-Wallis Statistics and P-values Indicating the Relationship Between Acc/F1 and instruction\_ft Across Datasets}
\begin{tabular}{lrl}
\toprule
dataset & statistic & pvalue \\
\midrule
agnews & 2.8318 & \textred{0.0924} \\
bbcnews & 1.3866 & 0.2390 \\
cdr & 0.3480 & 0.5553 \\
chemprot & 1.0168 & 0.3133 \\
ethos & 5.0521 & \textred{0.0246} \\
financial\_phrasebank & 0.1600 & 0.6892 \\
imdb & 3.4431 & \textred{0.0635} \\
semeval & 0.1882 & 0.6644 \\
sms & 0.3346 & 0.5630 \\
spouse & 1.3154 & 0.2514 \\
sst-2 & 0.2864 & 0.5925 \\
sst-5 & 0.3633 & 0.5467 \\
trec & 4.3282 & \textred{0.0375} \\
yelp & 2.6203 & 0.1055 \\
youtube & 2.2174 & 0.1365 \\
\bottomrule
\end{tabular}
\end{table}


==> results/per_datasets/tables/old/correlation_numparams_metric_spearman.tex <==
\begin{table}[h]
    \resizebox{\columnwidth}{!}{

\begin{tabular}{lcc}
\toprule
dataset & correlation coef & pvalue \\
\midrule
agnews & -0.1649 & 0.2003 \\
bbcnews & 0.0533 & 0.6660 \\
cdr & 0.2435 & \textred{0.0393} \\
chemprot & 0.1588 & 0.1826 \\
ethos & -0.2110 & 0.0751 \\
financial\_phrasebank & 0.0620 & 0.6051 \\
imdb & -0.2488 & 0.0512 \\
semeval & 0.0010 & 0.9936 \\
sms & 0.0950 & 0.4275 \\
spouse & 0.1039 & 0.3851 \\
sst-2 & 0.0548 & 0.6475 \\
sst-5 & -0.0008 & 0.9944 \\
trec & -0.1820 & 0.1568 \\
yelp & -0.0851 & 0.5107 \\
youtube & 0.1365 & 0.2529 \\
\bottomrule
\end{tabular}
    }
\caption{Spearman's Correlation Coefficients and P-values Indicating the Relationship Between Acc/F1 and num\_parameters Across Datasets}
\label{tab:correlation_numparams_metric}
\end{table}

